Partially-Typed NER Datasets Integration: Connecting Practice to Theory

While typical named entity recognition (NER) models require the training set to be annotated with all target types, each available datasets may only cover a part of them. Instead of relying on fully-typed NER datasets, many efforts have been made to leverage multiple partially-typed ones for training and allow the resulting model to cover a full type set. However, there is neither guarantee on the quality of integrated datasets, nor guidance on the design of training algorithms. Here, we conduct a systematic analysis and comparison between partially-typed NER datasets and fully-typed ones, in both theoretical and empirical manner. Firstly, we derive a bound to establish that models trained with partially-typed annotations can reach a similar performance with the ones trained with fully-typed annotations, which also provides guidance on the algorithm design. Moreover, we conduct controlled experiments, which shows partially-typed datasets leads to similar performance with the model trained with the same amount of fully-typed annotations

==> performance_all_cross.tex <==
\begin{table}[t]
\caption{Performance comparison on real-world datasets.}
\label{tab:cross_data}
\scalebox{0.9}{
\begin{tabular}{>{\centering}p{0.15cm}|c||c|ccc}
\hline
\multicolumn{2}{c||}{\textbf{Train set}} & \begin{tabular}[c]{@{}c@{}} \scriptsize BC4CHEMD, \\ \scriptsize NCBI-Disease\end{tabular} & \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}\scriptsize BC2GM , \\ \scriptsize BC4CHEMD \end{tabular}}
\\ \hline
\multicolumn{2}{c||}{\textbf{Test set}} & {\scriptsize BC5CDR}                                                            & \multicolumn{1}{c|}{\scriptsize Bio13PC}     & \multicolumn{1}{c|}{\scriptsize CRAFT}          & {\scriptsize Bio13CG }    \\ \hline\hline
M & \textit{\textbf{Cat}}  & 62.68                                                             & \multicolumn{1}{c|}{52.96}          & \multicolumn{1}{c|}{27.69}          & 38.00          \\
E & \textit{\textbf{Rnd}}     & 74.06                                                             & \multicolumn{1}{c|}{67.29}          & \multicolumn{1}{c|}{46.55}          & 73.16          \\
T & \textit{\textbf{Tok}}     & 75.16                                                             & \multicolumn{1}{c|}{67.16}          & \multicolumn{1}{c|}{45.97}          & 72.74          \\
H & \textit{\textbf{Ent}}     & 75.29                                                             & \multicolumn{1}{c|}{67.38}          & \multicolumn{1}{c|}{46.79}          & 73.75          \\ \cline{2-6}
O & \textit{\textbf{FuzzyNE}} & 65.36                                                             & \multicolumn{1}{c|}{64.96}          & \multicolumn{1}{c|}{39.68}          & 69.32          \\
D & \textit{\textbf{Fuzzy}}   & \textbf{77.50}                                                     & \multicolumn{1}{c|}{\textbf{69.34}} & \multicolumn{1}{c|}{\textbf{49.65}} & \textbf{74.18} \\ \hline
\end{tabular}}
\vspace{-0.3cm}
\end{table}

==> performance_all_full.tex <==

\begin{table*}[ht!]
\begin{center}
\small
\caption{Results on per-type in-corpus and cross-corpus F1. Model with $^*$ is trained on the single dataset.}
% \vspace{0.2cm}
\begin{tabularx}{\textwidth}{r | *{4}{Y} | *{8}{Y}}
% \hline
\toprule
% \begin{table*}[]
% \begin{tabular}{l||l|l|l|l|l|l|l|l|l|l|l|l}
% \hline \scriptsize
 & \multicolumn{4}{c|}{ In-corpus} & \multicolumn{8}{c}{Cross-corpus} \\ \midrule
% {\scriptsize Train Set} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\scriptsize BC4CHEMD & \scriptsize NCBI-Disease\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}} \scriptsize BC4CHEMD & \scriptsize BC2GM\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\scriptsize BC4CHEMD & \scriptsize NCBI-Disease\end{tabular}} & \multicolumn{6}{c}{\begin{tabular}[c]{@{}c@{}}\scriptsize BC4CHEMD & \scriptsize BC2GM\end{tabular}} \\ \midrule
\multirow{2}{*}{ Train Set} & \multicolumn{2}{c|}{\scriptsize BC4CHEMD} & \multicolumn{2}{c|}{\scriptsize BC2GM} & \multicolumn{2}{c|}{\scriptsize BC4CHEMD} & \multicolumn{6}{c}{\scriptsize BC2GM} \\ 
 & \multicolumn{2}{c|}{\scriptsize NCBI-Disease} & \multicolumn{2}{c|}{\scriptsize BC4CHEMD} & \multicolumn{2}{c|}{\scriptsize NCBI-Disease} & \multicolumn{6}{c}{\scriptsize BC4CHEMD} \\\midrule
{ Test Set} & \multicolumn{1}{c|}{\scriptsize BC4CHEMD} & \multicolumn{1}{c|}{\scriptsize NCBI-Disease} & \multicolumn{1}{c|}{\scriptsize BC2GM} & \multicolumn{1}{c|}{\scriptsize BC4CHEMD} & \multicolumn{2}{c|}{\scriptsize BC5CDR} & \multicolumn{2}{c|}{\scriptsize BioNLP13PC} & \multicolumn{2}{c|}{\scriptsize CRAFT} & \multicolumn{2}{c}{\scriptsize Bio13CG} \\ \midrule \midrule
% {\scriptsize Per-type F1} & {\scriptsize\texttt{CHEMICAL}} & {\scriptsize\texttt{DISEASE}} & {\scriptsize\texttt{PROTEIN}} & {\scriptsize\texttt{CHEMICAL}} & {\scriptsize\texttt{CHEMICAL}} & {\scriptsize\texttt{DISEASE}} & {\scriptsize\texttt{PROTEIN}} & {\scriptsize\texttt{CHEMICAL}} & {\scriptsize\texttt{PROTEIN}} & {\scriptsize\texttt{CHEMICAL}} & {\scriptsize\texttt{PROTEIN}} & {\scriptsize\texttt{CHEMICAL}} \\ \midrule \midrule
% \multirow{2}{*}{\small major of F1} & \texttt{\small CHEM} & \texttt{\small DISE} & \multirow{2}{*}{\texttt{\small PROTEIN}} &  \texttt{\small CHEM} & \texttt{\small CHEM} & \texttt{\small DISE} & \multirow{2}{*}{\texttt{\small PROTEIN}} & \texttt{\small CHEM} &  \multirow{2}{*}{\texttt{\small PROTEIN}} & \texttt{\small CHEM} &  \multirow{2}{*}{\texttt{\small PROTEIN}} & \texttt{\small CHEM} \\ 
%  & \texttt{\small ICAL} &\texttt{\small ASE} & &  \texttt{\small ICAL} &  \texttt{\small ICAL} & \texttt{\small ASE} & & \texttt{\small ICAL} & &  \texttt{\small ICAL} & & \texttt{\small ICAL}\\\midrule
\multirow{2}{*}{\small Metrics} & \texttt{\scriptsize CHEMIC} & \texttt{\scriptsize DISEA} & \texttt{\scriptsize PROTEIN} &  \texttt{\scriptsize CHEMIC} & \texttt{\scriptsize CHEMIC} & \texttt{\scriptsize DISEA} & \texttt{\scriptsize PROTEIN} & \texttt{\scriptsize CHEM} & \texttt{\scriptsize PROTEIN} & \texttt{\scriptsize CHEM} &  \texttt{\scriptsize PROTEIN} & \texttt{\scriptsize CHEM} \\ 
 & \texttt{\scriptsize -AL\_F1} &\texttt{\scriptsize -SE\_F1} & \texttt{\scriptsize \_F1} &  \texttt{\scriptsize -AL\_F1} &  \texttt{\scriptsize -AL\_F1} & \texttt{\scriptsize -SE\_F1} &  \texttt{\scriptsize \_F1} & \texttt{\scriptsize -AL\_F1} &  \texttt{\scriptsize \_F1} &  \texttt{\scriptsize -AL\_F1} &  \texttt{\scriptsize \_F1} & \texttt{\scriptsize -AL\_F1}\\\midrule
\textbf{\textit{Cat}} & 89.06 & 77.51 & 74.94 & 86.74 & 88.98 & 2.69 & 53.7 & 49.44 & 27.01 & 29.39 & 37.3 & 68.08 \\ \midrule
\textbf{\textit{Rnd}} & 88.93 & 82.80 & \textbf{79.93} & 87.23 & 87.99 & 55.05 & 69.22 & 58.57 & 48.84 & \textbf{39.68} & 72.68 & 74.84 \\ \midrule
\textbf{\textit{Tok}} & 89.23 & 82.51 & 78.51 & \textbf{89.16} & 88.90 & 56.20 & 68.75 & 60.07 & 49.05 & 36.86 & 72.53 & 73.46 \\ \midrule
\textbf{\textit{Ent}} & 88.93 & 82.76 & 79.83 & 87.98 & 89.27 & 56.01 & 49.65 & 38.10 & 49.65 & 38.10 & 73.77 & 73.69 \\ \midrule
\textbf{\textit{FuzzyNE}} & 82.14 & 81.67 & 78.51 & 87.79 & 90.05 & 12.41 & 65.81 & \textbf{61.28} & 40.05 & 38.79 & 67.15 & \textbf{76.29} \\ \midrule
\textbf{\textit{Fuzzy}} & \textbf{90.06} & \textbf{84.49} & 76.92 & 88.93 & \textbf{90.24} & \textbf{59.81} & \textbf{71.40} & 60.27 & \textbf{53.22} & 38.69 & \textbf{74.58} & 72.80 \\ \midrule
\textit{1-Type}$^*$ & 89.18 & 82.46 & 80.63 & 89.18 & 88.91 & 54.86 & 69.17 & 56.83 & 48.67 & 38.24 & 72.98 & 73.57 \\
% \end{tabular}
% \end{table*}
\bottomrule
\end{tabularx}
\end{center}
% assuming the vanilla LSTM to be adopted.}
\label{tab:pertype}
\end{table*}

==> statistics_all.tex <==
\begin{table}[t]
\begin{center}
\small
\caption{Data statistics. We show the number of sentences and the number of entity types with their counts of 3 train sets and 7 test sets.}
\label{tab:stats}
\scalebox{0.9}{
\begin{tabular}{p{1.9cm}|p{1.2cm}|p{4.2cm}}
\hline
\textbf{Name (train)} & \textbf{Sentences} & \textbf{Entity types and counts}\\
\hline
BC2GM & 15,092 & Protein (18,258)\\ %  (train0)
BC4CHEMD & 61,320 & Chemical (58,964) \\ % (train1)
NCBI-Disease & 6,347 & Disease (5,921) \\ % (train3)
\hline
\textbf{Name (test)} & \textbf{Sentences} & \textbf{Entity types and counts}\\
\hline
BC5CDR & 4,796 & Chemical(5,358), Disease(4,424)\\ % (test2)
BioNLP13PC & 1,694 & Protein(3,587), Chemical (858) \\
CRAFT & 7,424 & Protein(5,268), Chemical (2,169)\\
BioNLP13CG &1,905 & Protein(2,520), Chemical (727)\\
\hline
BC2GM & 5,037 & Protein(6,325) \\  %test0
BC4CHEMD & 26,363 & Chemical(25,346)\\  %test1
NCBI-Disease & 939 & Disease(960)\\ %test3
\hline
\end{tabular}}
\end{center}
\vsaft
\end{table}
